Long Short Term Memory Networks for Bandwidth Forecasting in Mobile Broadband Networks under Mobility

Bandwidth forecasting in Mobile Broadband (MBB) networks is a challenging task, particularly when coupled with a degree of mobility. In this work, we introduce HINDSIGHT++, an open-source R-based framework for bandwidth forecasting experimentation in MBB networks with Long Short Term Memory (LSTM) networks. We instrument HINDSIGHT++ following an Automated Machine Learning (AutoML) paradigm to first, alleviate the burden of data preprocessing, and second, enhance performance related aspects. We primarily focus on bandwidth forecasting for Fifth Generation (5G) networks. In particular, we leverage 5Gophers, the first open-source attempt to measure network performance on operational 5G networks in the US. We further explore the LSTM performance boundaries on Fourth Generation (4G) commercial settings using NYU-METS, an open-source dataset comprising of hundreds of bandwidth traces spanning different mobility scenarios. Our study aims to investigate the impact of hyperparameter optimization on achieving state-of-the-art performance and beyond. Results highlight its significance under 5G scenarios showing an average Mean Absolute Error (MAE) decrease of near 30% when compared to prior state-of-the-art values. Due to its universal design, we argue that HINDSIGHT++ can serve as a handy software tool for a multitude of applications in other scientific fields.

==> Sections/HINDSIGHT/timelags.tex <==
\subsection{AutomaL: Toward Automating Lags Selection}
\label{sec:timelags}

As their name imply, \ac{LSTM} networks were designed to address the problem of long-term dependencies in sequential data that \ac{RNN} were unable to deal with.
To capture such dependencies, it is critical that the length of the input sequence, widely know in the literature as \textit{lags}, is properly defined.
%\footnote{The terms \textit{time lags} or \textit{lags} will be from now on used interchangeably.}.
In other words, lags constitute the lookback  window that will be used during the next prediction step (or steps), therefore, its selection can greatly affect model's efficiency.
However, it is rarely intuitive on how to select the optimal value or with which criteria, since it highly relies on the nature of the data and the problem under study.
For example, in text recognition, where learning long-term dependencies is crucial, a large window is usually favored.
It is worth mentioning that a single lag will result to what is called the \textit{persistence model}, which is often considered as the baseline. 
A model is called persistence when the output predictions are tightly coupled with the previous values.
From a mathematical point of view, such a model can be expressed as $P(t+1) = P(t)$, where $P$ represents the predicted outcome at each time frame.
To the best of our knowledge, a systematic approach that dynamically dictates the optimal lags value by considering explicit characteristics of the input data, such as periodic patterns and/or repetitions, has not yet been proposed in the literature.

We introduce \emph{AutomaL}, a novel algorithm that automates the lags selection process by combining state-of-the-art statistical concepts, such as stationarity and autocorrelation, and serves as an optimization step prior to the model design.
%An overview of the main blocks of the algorithm can be depicted in Figure \ref{figure:lags}.
Listing \ref{alg:lags} provides an overview of the algorithm's main blocks outlined in a pseudocode fashion.
As an initial step, we perform a stationarity test on the target sequence by leveraging the Dickey-Fuller test.
To reduce or even remove the effect of potential diverse variances, trend components and seasonality, we consider a transformed version of the data by applying a logarithmic scale and differencing, i.e., we subtract the previous sample from the current sample.
The null hypothesis that the unit root is present in the data is rejected with a $95\%$ (i.e., default) \ac{CI} (i.e., $p-value<0.05$).
If so, the alternative hypothesis takes place and the sequence is marked as stationary\footnote{Even though a stationary sequence can contribute to the model's predictive performance, it is not by any means an \ac{LSTM} hard requirement. Thus said, for non-stationary data, the default lags value is used instead.}.
Consequently, we proceed by calculating the auto-correlation function, that in turn, reveals the presence of repeating or periodic patterns.
Last, we use a peak detection algorithm found in  \cite{peakdetection} to discover all available peaks\footnote{The \texttt{findPeaks} function features an input parameter $m$, that is used to adjust the sensitivity of the peak detection process. Since the only way to verify that the algorithm is not over (or even under) detecting peaks or valleys is by using visualization evidence, we select its value based on sensitivity analysis means (i.e., $m=1$).}
%we select a value based on the default value that provides a compromise between the two.}.
\emph{AutomaL} uses the first detected peak to determine the number of lags and returns it back to the main function.
Similar to feature selection, for parallel forecasting tasks and given that lags vary across the target sequences, we adopt a majority-voting strategy.
% a \textit{NULL} value is returned instead, and the user is prompted to manually assign a value.\kostas{Check this one}
%Alternatively, the user is given the option to treat lags as a hyperparameter, thus, its value will be selected during the hyperparameter optimization phase, as we will explain in a later subsection.\kostas{manual or AutomaL is implemented}
%It is noteworthy to add that the latter case will significantly increase the running time computational complexity.

\textit{Discussion and considerations:} We tested \emph{AutomaL} with a variety of time series datasets. 
When seasonal trends with periodic cycles are prominent in the data (i.e., with visual inspection or even mathematical evidence), \emph{AutomaL} determines, or closely approaches, a near-optimum lags value. 
However, different hyperparameter configurations can significantly affect the predictive error, hence, \emph{AutomaL}'s output should be treated as a recommendation, rather than an optimal value\footnote{A recommendation tag precedes the output value to accentuate our statement.}.
Furthemore, datasets with no seasonal components may not benefit from \emph{AutomaL}, therefore, a different tuning approach (e.g., Random search optimization) could be used as an alternative.

% \begin{figure}[h!]
%   \centering
%     \includegraphics[keepaspectratio,width = 0.9\linewidth]{img/lags.pdf} 
%       \caption{An abstract representation of the main blocks that comprise \emph{AutomaL}.}
%   \label{figure:lags}
% \end{figure}

\begin{algorithm}
  \caption{\small \emph{AutomaL}: A systematic approach to automate the lags selection.}
  \label{alg:lags}
  \begin{algorithmic}[1]
      \Require target sequence(s)
      \Ensure lags 
      \State stat = adf.test(target) \qquad \#Stationarity test
      \If {target sequence is stationary}
          \State auto = acf(target) \qquad \#Autocorrelation calculation
          \State findPeaks(auto, m) \qquad \#Peak Detection
          \State lags = First Peak \qquad \# Determine lags 
      \Else
         \State lags = default value
      \EndIf
      \State Return lags
  \end{algorithmic}
\end{algorithm}



==> Sections/related.tex <==
\section{Related Work}
\label{sec:related}

In this section, we summarize related literature on bandwidth forecasting and report additional work on  \ac{LSTM} applications.

\textbf{Bandwidth Forecasting:} 
Bandwidth forecasting is a challenging and rather critical process for a plethora of applications and tasks including network performance optimization, traffic management, application provisioning, and crowdsourced reporting. 
Over the years, several studies have attempted to model or predict the performance of \ac{MBB} networks.
Even though most of these studies tackle the problem from separate angles, they share a common objective, i.e., to minimize the error function and provide insights on the complexity of the mobile ecosystem.

A supervised \ac{ML} solution for downlink throughput prediction in \ac{MBB} networks is proposed in \cite{Kousias2019}.
The authors show that \ac{ML} can significantly reduce the data volume consumption over the network, while maintaining the predictive error in acceptable levels. 
Furthermore, Raida et. al in \cite{raida2018constant} leverage constant rate probing packets for a very short duration to estimate available bandwidth in a controlled \ac{LTE} environment, while in \cite{raida2019constant} the authors extend their work by further testing and validating the developed framework in live \ac{LTE} networks.
In \cite{Maier2019}, Maier et al. introduce a novel \ac{AI} model that leverages feed-forward neural networks for downlink and uplink bandwidth forecasting.
To find a fitting speed test duration, the authors investigate two scenarios.
First, they train a model with a duration fixed to a value lower than default, while second, they dynamically determine a duration by using the results of a pretrained neural network model. 
Experimental approaches studying the problem of bandwidth prediction have also been addressed in  \cite{liu2015empirical, mirza2007machine, samba2017instantaneous, wei2018trust, riihijarvi2018machine, linder2016using, rattaro2010throughput}.
Beyond empirical-based studies, theoretical models have also been studied.
In \cite{gao2018prophet}, Gao et al. introduce a theoretical learning based throughput prediction system for reactive flows, while authors in \cite{bui2014model} propose a novel stochastic model for user throughput prediction in \ac{MBB} networks that considers fast fading and user location. 

In addition, several works that focus on network performance prediction using \ac{LSTM} networks have been recently proposed.
Most notably, the authors in \cite{mei2019realtime} address a real-time bandwidth prediction problem by leveraging \ac{LSTM}-based prediction models, while in \cite{cui2018deep}, Cui et al. propose a stacked bidirectional \ac{LSTM} architecture for network-wide traffic estimation.
Furthermore, Zhao et. al. in \cite{zhao2017lstm} focus on a short-term traffic estimation problem by considering temporal–spatial correlation, whereas, authors in \cite{wang2017spatiotemporal} propose a hybrid framework that combines \ac{LSTM} networks and an auto-encoder based model for solving a spatio-temporal prediction problem.

Next, we argue how our work stands out and distinguishes itself from state-of-the-art research. 
Despite the fact that the previous studies make use of \ac{LSTM} networks for modeling different aspects of the network, they do not explore the potential of hyperparameter optimization toward improving their  performance. 
In addition, to the best of our knowledge, this is the first large-scale study that attempts to perform a comparative bandwidth forecasting analysis between \ac{4G} and \ac{5G} operational networks under various mobility scenarios. 
Last, we make available to the community an open-source framework which follows an end-to-end \ac{AutoML} paradigm and allows for ample experimentation with \ac{LSTM} networks.

%\textbf{\ac{LSTM} applications:} 
% Since \ac{LSTM} networks were explicitly designed to handle long-term dependencies, they have found applicability in a plethora of problems that require long range memory, such as reinforcement learning \cite{bakker2002reinforcement}, handwriting recognition \cite{pham2014dropout,graves2005framewise,sun2016deep,wigington2017data}, text classification \cite{nowak2017lstm}, speech and voice recognition \cite{graves2013hybrid,tilk2015lstm,graves2004biologically,lehner2015low}, acoustic and language modeling \cite{sak2014long,sundermeyer2015feedforward,schmidhuber2002learning}, audio and video analysis \cite{marchi2014multi,donahue2015long}, malware and anomaly detection \cite{vinayakumar2018detecting,malhotra2015long,chauhan2015anomaly}, medical and clinical related studies \cite{lipton2015phenotyping,liu2016augmented}, as well as a wider range of tasks that require precise timing \cite{gers2002learning,lipton2015learning,filonov2016multivariate}.


